Exploring the Benefits of Domain-Pretraining of Generative Large Language Models for Chemistry

A proliferation of Large Language Models (the GPT series, BLOOM, LLaMA, and more) are driving forward novel development of multipurpose AI for a variety of tasks, particularly natural language processing (NLP) tasks. These models demonstrate strong performance on a range of tasks; however, there has been evidence of brittleness when applied to more niche or narrow domains where hallucinations or fluent but incorrect responses reduce performance. Given the complex nature of scientific domains, it is prudent to investigate the trade-offs of leveraging off-the-shelf versus more targeted foundation models for scientific domains. In this work, we examine the benefits of in-domain pre-training for a given scientific domain, chemistry, and compare these to open-source, off-the-shelf models with zero-shot and few-shot prompting. Our results show that not only do in-domain base models perform reasonably well on in-domain tasks in a zero-shot setting but that further adaptation using instruction fine-tuning yields impressive performance on chemistry-specific tasks such as named entity recognition and molecular formula generation.

==> figures/entity_subtask_perf.tex <==
\pgfplotstableread{ 
% model performance per entity type for entity extraction
%index entitytype 	AISLE GPT2-XL	AISLE BLOOM-3B	BASELINE GPT2-XL	BASELINE BLOOM-3B
index entitytype 	{AG0}	{AB0}	{BG0} 	{BB0}
1 ABBREVIATION	 0.009800	0.004872	0.003232	0.005794
2 FAMILY	     0.534315	0.417408	0.514815	0.486771
3 FORMULA	     0.007222	0.001856	0.003490	0.008557
4 IDENTIFIER	 0.004255	0.004474	0.003953	0.006263
5 MULTIPLE	     0.139690	0.150602	0.132432	0.105381
6 SYSTEMATIC	 0.517792	0.357456	0.534311	0.508735
7 TRIVIAL	     0.553085	0.356504	0.576681	0.515585
}\dfcee

%ABBREVIATION (Abbr.),  FAMILY   (Fam.), FORMULA   (Form.), IDENTIFIER  (Ident.), MULTIPLE     (Multi.), SYSTEMATIC    (Syst.) , TRIVIAL        (Triv.) , and overall     


\pgfplotstableread{ 
% model performance per entity type for entity recognition (cer)
%index entitytype MAI GPT2-XL	MAI BLOOM-3B	BASELINE GPT2-XL	BASELINE BLOOM-3B
index entitytype {AG0}	{AB0}	{BG0}	{BB0}
1 ABBREVIATION	0.833424	0.247744	0.803190	0.838230
2 FAMILY	    0.817140	0.326045	0.793220	0.806050
3 FORMULA	    0.810533	0.297561	0.815912	0.788765
4 IDENTIFIER	0.773694	0.242706	0.731614	0.770149
5 MULTIPLE	    0.679852	0.210181	0.696759	0.680488
6 SYSTEMATIC	0.825707	0.317912	0.810761	0.827721
7 TRIVIAL	    0.858375	0.386719	0.823759	0.842175
}\dfcer


  \pgfplotsset{every tick label/.append style={font=\tiny, xshift=0.5ex}}
    \begin{tikzpicture} 
    \begin{axis}[ 
    %xlabel=Exam Topic(s),
    ylabel={\textbf{CER}\\F1},
    ylabel style = {align=center},  
    %title={\textit{CER}},
    %title style = {align = center}, 
    %title style={at={(current bounding box.north west)}, anchor=south west},
title style = {yshift=-0.1in}, 
   % ylabel style = {yshift=-0.2in},  
    %title style = {yshift=-0.1in},
    height=2.75cm,%3cm,
    %ytick={0,0.25,0.5,0.75,1},
    width=16cm, 
    bar width=9,
    axis lines=left,
    xmin=0.5,
    xmax=7.5,
        %        xscale = 0.75, 
        %        yscale=0.5, 
        %xbar stacked,
        ybar,
        ymin=0, 
        ymax=1,
        xtick=data,
        font=\footnotesize,
        xticklabels from table={\dfcer}{entitytype},
        %yticklabel style={text width=2cm,align=center},
        legend columns=4,
        legend style={at={(0.5,-0.45)},anchor=north,draw=none,
    column sep=0.75ex,}
    ]    
    \addplot+[color=aisleGPT] table [x=index, meta=entitytype, y= AG0] {\dfcer}; 
    %\addlegendentry{AISLE GPT2-XL}% (3)}
    \addplot+[color=aisleBloom] table [x=index, meta=entitytype, y= AB0] {\dfcer};
    %\addlegendentry{AISLE Bloom-3B}% (3)}
    \addplot+[color=baseGPT,] table [x=index, meta=entitytype, y= BG0] {\dfcer}; 
    %\addlegendentry{Baseline GPT2-XL}% (3)}
    \addplot+[color=baseBloom] table [x=index, meta=entitytype, y= BB0] {\dfcer}; 
    %\addlegendentry{Baseline Bloom-3B}% (3)}
    \end{axis}
    \end{tikzpicture} 
    
  %\centering
  \pgfplotsset{every x tick label/.append style={font=\tiny, xshift=0.5ex}}
  \pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.5ex}}
    \begin{tikzpicture} 
    \begin{axis}[ 
    %xlabel=Exam Topic(s),
    ylabel={\textbf{CEE}\\F1},
    ylabel style = {align=center}, 
    %title={\textit{CEE}},
    %title style = {align = center}, 
    %title style={at={(current bounding box.north west)}, anchor=south west},
    %title style = {yshift=-0.1in},  
    %ylabel style = {yshift=-0.2in}, 
    %title style = {yshift=-0.1in},
    height=3cm,
    width=16cm, 
    bar width=9,
    axis lines=left,
    xmin=0.5,
    xmax=7.5,
        %        xscale = 0.75, 
        %        yscale=0.5, 
        %xbar stacked,
        ybar,
        ymin=0,
        ymax=1,
        xtick=data,
        font=\footnotesize,
        xticklabels from table={\dfcee}{entitytype}, 
        %yticklabel style={text width=2cm,align=center},
        legend columns=4,
        legend style={at={(0.5,-0.45)},anchor=north,draw=none,
    column sep=0.75ex,}
    %xticklabels={,,,,,,,,},
    ]
    \addplot+[color=aisleGPT] table [x=index, meta=entitytype, y= AG0] {\dfcee}; 
    \addlegendentry{AISLE GPT2-XL}% (0)}
    \addplot+[color=aisleBloom] table [x=index, meta=entitytype, y= AB0] {\dfcee}; 
    \addlegendentry{AISLE Bloom-3B}% (0)}
    \addplot+[color=baseGPT] table [x=index, meta=entitytype, y= BG0] {\dfcee}; 
    \addlegendentry{Baseline GPT2-XL}% (0)}
    \addplot+[color=baseBloom] table [x=index, meta=entitytype, y= BB0] {\dfcee}; 
    \addlegendentry{Baseline Bloom-3B}% (0)}

    
    %\addplot+ table [x=index, meta=Subset, y= BG3] {\df}; 
    %\addlegendentry{Baseline GPT2-XL (3)}
    %\addplot+ table [x=index, meta=Subset, y= BB3] {\df}; 
    %\addlegendentry{Baseline Bloom-3B (3)}
    %\addplot+ table [aisleGPT, x=index, meta=Subset, y= AG3] {\df}; 
    %\addlegendentry{AISLE GPT2-XL (3)}
    %\addplot+ table [aisleBloom,x=index, meta=Subset, y= AB3] {\df};
    %\addlegendentry{AISLE Bloom-3B (3)}
    
    \end{axis}
    \end{tikzpicture}
     \vspace{-.75\baselineskip}


 

==> figures/treemap_chemistry.tex <==
\begin{tabular}{c} 
\begin{tikzpicture}[ 
                xscale = 0.95,%1.4, 
                yscale=0.7,%0.75, 
                font=\sffamily\tiny,
                mystyle/.style={draw=white, very thick, text=white, font=\sffamily\bfseries\small}
                ]
        \pie[hide number,square,  
              style={mystyle}, 
              color= {AminerColor,MagColor,S2OrcColor,WosColor,ArxivColor, DblpColor, OstiColor, PubmedColor,Cord19Color}, % e.g. {colorOne, colorTwo}, %do not use _ in color names
              %text=inside, %include text in tree map bars
              %text=legend, %include text as a legend
              %text=None, % don't include the text 
              text=pin
              ]{
              56.27/AMiner,
              33.93/MAG,
              4.54/S2ORC,
              4.32/WoS,
              0.4/arXiv,
              0.2/DBLP,
              0.1/OSTI,
              0.04/PubMed,
              0.01/CORD19
              }
  %{ 
		% 32.23/MAG,
		% 18.96/CORE,
		% 17.44/AMiner,
		% 12.19/WoS,
		% 10.73/PubMed,
		% 5.59/S2ORC,
		% 1.53/OSTI,
		% 1.26/arXiv~~~~~~,
		% 0.04/CORD19 (.05\%),
		% 0.03/DBLP (.03\%),
		% 0.0/~~~~~~~ ~~~~~~~~~~~~bioRxiv (<0.01\%) %(0.005\%)
		% }
		
           % \node[above,font=\small\bfseries] at (current bounding box.north) {Chemistry Data Sources (after deduplication)};
\end{tikzpicture}
\end{tabular}



==> tables.tex <==

% Chemistry, Science, Language (acc) - Zero-shot
\begin{tabular}{lrr|rrrrr|rrrrr}
\toprule
Zero-shot (acc) &     HT-HC &  HT-CC &     ARC-E &     ARC-C &   SciQ &  OpenBookQA &    MathQA &        CB &     BoolQ &       WSC &       WIC &      PIQA \\
\midrule
Instruction Fine-tuned BASELINE BLOOM-3B &  0.251232 &   0.29 &  0.343013 &  0.203925 &  0.587 &       0.168 &  0.201340 &  0.500000 &  0.378287 &  0.634615 &  0.500000 &  0.563656 \\
Instruction Fine-tuned MAI GPT2-XL       &  0.216749 &   0.35 &  0.430135 &  0.225256 &  0.686 &       0.198 &  0.201675 &  0.500000 &  0.378287 &  0.634615 &  0.500000 &  0.555495 \\
Instruction Fine-tuned MAI BLOOM-3B      &  0.226601 &   0.36 &  0.402357 &  0.220990 &  0.703 &       0.170 &  0.221776 &  0.482143 &  0.402752 &  0.451923 &  0.500000 &  0.560936 \\
Instruction Fine-tuned BASELINE GPT2-XL  &  0.231527 &   0.26 &  0.431818 &  0.213311 &  0.729 &       0.192 &  0.201675 &  0.500000 &  0.432416 &  0.509615 &  0.485893 &  0.626224 \\
From Scratch MAI GPT2-XL                 &  0.266010 &   0.31 &  0.496633 &  0.215017 &  0.803 &       0.194 &  0.230486 &  0.250000 &  0.464832 &  0.365385 &  0.501567 &  0.596844 \\
From Scratch MAI BLOOM-3B                &  0.206897 &   0.26 &  0.485269 &  0.221843 &  0.799 &       0.182 &  0.217755 &  0.107143 &  0.383180 &  0.538462 &  0.514107 &  0.579434 \\
From Scratch BASELINE GPT2-XL            &  0.182266 &   0.26 &  0.582912 &  0.250853 &  0.832 &       0.224 &  0.235846 &  0.071429 &  0.614679 &  0.500000 &  0.498433 &  0.708379 \\
From Scratch BASELINE BLOOM-3B           &  0.226601 &   0.23 &  0.594697 &  0.279863 &  0.892 &       0.216 &  0.249581 &  0.410714 &  0.620795 &  0.375000 &  0.498433 &  0.707835 \\
\bottomrule
\end{tabular}

% Chemistry, Science, Language (acc) - Three-shot
\begin{tabular}{lrr|rrrrr|rrrrr}
\toprule
Three-Shot (acc) &     HT-HC &  HT-CC &     ARC-E &     ARC-C &   SciQ &  OpenBookQA &    MathQA &        CB &     BoolQ &       WSC &       WIC &      PIQA \\
\midrule
Instruction Fine-tuned MAI GPT2-XL       &  0.221675 &   0.35 &  0.424663 &  0.228669 &  0.672 &       0.196 &  0.204355 &  0.607143 &  0.423547 &  0.365385 &  0.518809 &  0.544070 \\
Instruction Fine-tuned MAI BLOOM-3B      &  0.275862 &   0.30 &  0.414141 &  0.209898 &  0.722 &       0.180 &  0.206365 &  0.464286 &  0.466361 &  0.365385 &  0.517241 &  0.570185 \\
Instruction Fine-tuned BASELINE GPT2-XL  &  0.201970 &   0.31 &  0.422138 &  0.227816 &  0.714 &       0.190 &  0.207035 &  0.482143 &  0.399083 &  0.605769 &  0.489028 &  0.636017 \\
Instruction Fine-tuned BASELINE BLOOM-3B &  0.251232 &   0.34 &  0.333333 &  0.208191 &  0.555 &       0.164 &  0.196650 &  0.500000 &  0.379511 &  0.557692 &  0.495298 &  0.556583 \\
From Scratch MAI GPT2-XL                 &  0.270936 &   0.36 &  0.458333 &  0.215870 &  0.800 &       0.180 &  0.222446 &  0.446429 &  0.526911 &  0.365385 &  0.510972 &  0.591404 \\
From Scratch MAI BLOOM-3B                &  0.246305 &   0.35 &  0.469276 &  0.226962 &  0.801 &       0.182 &  0.220101 &  0.357143 &  0.495413 &  0.365385 &  0.507837 &  0.598477 \\
From Scratch BASELINE GPT2-XL            &  0.201970 &   0.25 &  0.587963 &  0.258532 &  0.893 &       0.234 &  0.242211 &  0.285714 &  0.617125 &  0.365385 &  0.492163 &  0.704026 \\
From Scratch BASELINE BLOOM-3B           &  0.231527 &   0.28 &  0.632997 &  0.319966 &  0.934 &       0.234 &  0.250251 &  0.517857 &  0.622324 &  0.365385 &  0.496865 &  0.711643 \\
\bottomrule
\end{tabular}

% Perplexity Tasks (ppl) - 0-shot
\begin{tabular}{lrrrr}
\toprule
Zero-Shot (acc) &  OpenAI Lambada &  Wikitext2 Raw &  Pile Abstracts &  Core Abstracts \\
\midrule
Instruction Fine-tuned MAI GPT2-XL       &    1.788815e+04 &     946.980309 &      250.101930 &             NaN \\
Instruction Fine-tuned MAI BLOOM-3B      &    3.124881e+03 &     474.219605 &      222.586400 &             NaN \\
Instruction Fine-tuned BASELINE GPT2-XL  &    2.334898e+02 &     128.091156 &      746.182436 &             NaN \\
Instruction Fine-tuned BASELINE BLOOM-3B &    1.333980e+06 &    3067.969323 &     2332.866789 &             NaN \\
From Scratch MAI GPT2-XL                 &    3.333900e+02 &      89.647906 &       25.251878 &      246.853606 \\
From Scratch MAI BLOOM-3B                &    1.932161e+02 &      69.336140 &       21.657962 &      223.216635 \\
From Scratch BASELINE GPT2-XL            &    1.063501e+01 &      20.376518 &       42.292437 &      234.463318 \\
From Scratch BASELINE BLOOM-3B           &    9.094238e+00 &      31.071619 &       24.208852 &      160.670023 \\
\bottomrule
\end{tabular}

% HT-HC Accuracy
\begin{tabular}{lrr}
\toprule
hendrycksTest-high\_school\_chemistry &       Base &  +Instruction \\
\midrule
MAI GPT2-XL       &  26.600985 &     21.674877 \\
MAI BLOOM-3B      &  20.689655 &     22.660099 \\
\midrule
BASELINE GPT2-XL  &  18.226601 &     23.152709 \\
BASELINE BLOOM-3B &  22.660099 &     25.123153 \\
\bottomrule
\end{tabular}


